The Impact of Quantization on Large Reasoning Model Reinforcement Learning

Strong reasoning capabilities can now be achieved by large-scale reinforcement learning (RL) without any supervised fine-tuning. Although post-training quantization (PTQ) and quantization-aware training (QAT) are well studied in the context of fine-tuning, how quantization impacts RL in large reasoning models (LRMs) remains an open question. To answer this question, we conducted systematic experiments and discovered a significant gap in reasoning performance on mathematical benchmarks between post-RL quantized models and their quantization-aware RL optimized counterparts. Our findings suggest that quantization-aware RL training negatively impacted the learning process, whereas PTQ and QLoRA led to greater performance.

==> main_table_copy.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|l|c|c|c|l|l|c|}
        \hline
        \multirow{2}{*}{Model} &
        \multicolumn{4}{c|}{Qwen} \\
         & $0.6$B & $1.7$B & $4$B & $8$B\\      \hline  
        (Base) &0.1644  & 0.2115& 0.4511&0.4733 \\
        \hline
        (GRPO) &0.3066 &0.4176  &0.5544 & 0.5938\\
        (drGRPO) &0.2430  & 0.2845& 0.5412 & 0.5840 \\
        \hline 
        (STE 8-bit)  &0.2417  &0.3252  & 0.4438 & 0.4964  \\
        (PTQ BnB 8-bit) &0.2216 & 0.3662& 0.5276&0.5792 \\
        (PTQ AWQ 8-bit) &0.2200 & 0.3644&0.5264 & 0.5831\\
        \hline 
        (QLoRA 4-bit) &0.2715 & 0.3819& 0.5544 & 0.5563 \\
        (PTQ BnB 4-bit) & 0.2228&0.3686 & 0.5270& 0.5805\\
        (PTQ AWQ 4-bit) &0.2248 &0.3656 & 0.5328& 0.5736\\
        \hline
    \end{tabular}
    \caption{Mean reward (rounded to 4 decimal places)}
    \label{tab:evaluation_math} 
\end{table}
